MIMO Networks: the Effects of Interference

Multiple-input/multiple-output (MIMO) systems promise enormous capacity increase and are being considered as one of the key technologies for future wireless networks. However, the decrease in capacity due to the presence of interferers in MIMO networks is not well understood. In this paper, we develop an analytical framework to characterize the capacity of MIMO communication systems in the presence of multiple MIMO co-channel interferers and noise. We consider the situation in which transmitters have no information about the channel and all links undergo Rayleigh fading. We first generalize the known determinant representation of hypergeometric functions with matrix arguments to the case when the argument matrices have eigenvalues of arbitrary multiplicity. This enables the derivation of the distribution of the eigenvalues of Gaussian quadratic forms and Wishart matrices with arbitrary correlation, with application to both single user and multiuser MIMO systems. In particular, we derive the ergodic mutual information for MIMO systems in the presence of multiple MIMO interferers. Our analysis is valid for any number of interferers, each with arbitrary number of antennas having possibly unequal power levels. This framework, therefore, accommodates the study of distributed MIMO systems and accounts for different positions of the MIMO interferers.

==> figures/figscenario.tex <==
%TeXCAD Options
%\grade{\on}
%\emlines{\off}
%\beziermacro{\on}
%\reduce{\on}
%\snapping{\on}
%\quality{8}
%\graddiff{.01}
%\snapasp{1}
%\zoom{6.7271}
\unitlength 0.90mm % = 2.85pt
\linethickness{0.4pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi % GNUPLOT compatibility
\begin{picture}(89,107)(0,0)
\put(10.2,103.4){\line(1,0){8}}
\put(22.2,106.4){\line(0,-1){6}}
\put(15.2,82.4){\makebox(0,0)[cc]{$\Nt_0$}}
\put(18.2,103.4){\line(4,3){4}}
\put(18.2,103.4){\line(4,-3){4}}
\put(10.45,88.15){\line(1,0){8}}
\put(18.45,88.15){\line(4,3){4}}
\put(14.95,95.65){\oval(2.5,19.5)[]}
%\emline(18.55,87.99)(22.44,85.52)
\multiput(18.55,87.99)(.0525676,-.0333784){74}{\line(1,0){.0525676}}
%\end
%\emline(22.44,85.52)(22.44,90.82)
\put(22.44,85.52){\line(0,1){5.3}}
%\end
\put(78,87.12){\line(-1,0){8}}
\put(78,103.12){\line(-1,0){8}}
\put(66,84.12){\line(0,1){6}}
\put(66,100.12){\line(0,1){6}}
\put(74,82.12){\makebox(0,0)[]{$\Nr$}}
\put(70,87.12){\line(-4,-3){4}}
\put(70,103.12){\line(-4,-3){4}}
\put(70,87.12){\line(-4,3){4}}
\put(70,103.12){\line(-4,3){4}}
\put(73.25,94.87){\oval(2.5,19.5)[]}
\put(4,94){\makebox(0,0)[cc]{$\Pt_0, \ \x_0$}}
\put(38,96){\makebox(0,0)[cc]{$\H_0$}}
\put(37,73){\makebox(0,0)[cc]{$\H_1$}}
\put(38,34){\makebox(0,0)[cc]{$\H_{\Ni}$}}
%\vector(44,96)(55,96)
\put(55,96){\vector(1,0){.07}}
\put(44,96){\line(1,0){11}}
%\end
%\vector(27,67)(32,70)
\put(32,70){\vector(3,2){.07}}
\multiput(27,67)(.0561798,.0337079){89}{\line(1,0){.0561798}}
%\end
%\vector(43,76)(51,81)
\put(51,81){\vector(3,2){.07}}
\multiput(43,76)(.05369128,.03355705){149}{\line(1,0){.05369128}}
%\end
%\vector(26,19)(32,26)
\put(32,26){\vector(3,4){.07}}
\multiput(26,19)(.03370787,.03932584){178}{\line(0,1){.03932584}}
%\end
%\vector(44,40)(55,57)
\put(55,57){\vector(2,3){.07}}
\multiput(44,40)(.033639144,.051987768){327}{\line(0,1){.051987768}}
%\end
\put(89,94){\makebox(0,0)[cc]{$\y$}}
\put(10.2,25){\line(1,0){8}}
\put(10.2,73){\line(1,0){8}}
\put(22.2,28){\line(0,-1){6}}
\put(22.2,76){\line(0,-1){6}}
\put(15.2,4){\makebox(0,0)[cc]{$\Nt_{\Ni}$}}
\put(15.2,52){\makebox(0,0)[cc]{$\Nt_1$}}
\put(18.2,25){\line(4,3){4}}
\put(18.2,73){\line(4,3){4}}
\put(18.2,25){\line(4,-3){4}}
\put(18.2,73){\line(4,-3){4}}
\put(10.45,9.75){\line(1,0){8}}
\put(10.45,57.75){\line(1,0){8}}
\put(18.45,9.75){\line(4,3){4}}
\put(18.45,57.75){\line(4,3){4}}
\put(14.95,17.25){\oval(2.5,19.5)[]}
\put(14.95,65.25){\oval(2.5,19.5)[]}
%\emline(18.55,9.59)(22.44,7.12)
\multiput(18.55,9.59)(.0525676,-.0333784){74}{\line(1,0){.0525676}}
%\end
%\emline(18.55,57.59)(22.44,55.12)
\multiput(18.55,57.59)(.0525676,-.0333784){74}{\line(1,0){.0525676}}
%\end
%\emline(22.44,7.12)(22.44,12.42)
\put(22.44,7.12){\line(0,1){5.3}}
%\end
%\emline(22.44,55.12)(22.44,60.42)
\put(22.44,55.12){\line(0,1){5.3}}
%\end
\put(4,15.6){\makebox(0,0)[cc]{$\Pt_{\Ni}, \ \x_{\Ni}$}}
\put(4,63.6){\makebox(0,0)[cc]{$\Pt_1, \ \x_1$}}
\put(15,45){\circle*{0}}
\put(15,41){\circle*{2}}
\put(15,36){\circle*{2}}
\put(15,45){\circle*{2}}
\put(80,103){\circle{2.83}}
\put(80,87){\circle{2.83}}
%\emline(80,104)(80,102)
\put(80,104){\line(0,-1){2}}
%\end
%\emline(80,88)(80,86)
\put(80,88){\line(0,-1){2}}
%\end
%\emline(80,102)(80,102)
\put(80,102){\line(0,1){0}}
%\end
%\emline(80,86)(80,86)
\put(80,86){\line(0,1){0}}
%\end
%\emline(80,102)(80,102)
\put(80,102){\line(0,1){0}}
%\end
%\emline(80,86)(80,86)
\put(80,86){\line(0,1){0}}
%\end
%\emline(79,103)(81,103)
\put(79,103){\line(1,0){2}}
%\end
%\emline(79,87)(81,87)
\put(79,87){\line(1,0){2}}
%\end
%\emline(81,103)(84,103)
\put(81,103){\line(1,0){3}}
%\end
%\emline(81,87)(84,87)
\put(81,87){\line(1,0){3}}
%\end
%\emline(79,107)(79,107)
\put(79,107){\line(0,1){0}}
%\end
%\vector(80,98)(80,101)
\put(80,101){\vector(0,1){.07}}
\put(80,98){\line(0,1){3}}
%\end
%\vector(80,82)(80,85)
\put(80,85){\vector(0,1){.07}}
\put(80,82){\line(0,1){3}}
%\end
\put(80,78){\makebox(0,0)[cc]{$\n$}}
%\vector(27,96)(33,96)
\put(33,96){\vector(1,0){.07}}
\put(27,96){\line(1,0){6}}
%\end
\end{picture}

